Public-Key Based Authentication Architecture for IoT Devices Using PUF

Nowadays, Internet of Things (IoT) is a trending topic in the computing world. Notably, IoT devices have strict design requirements and are often referred to as constrained devices. Therefore, security techniques and primitives that are lightweight are more suitable for such devices, e.g., Static Random-Access Memory (SRAM) Physical Unclonable Functions (PUFs) and Elliptic Curve Cryptography (ECC). SRAM PUF is an intrinsic security primitive that is seeing widespread adoption in the IoT segment. ECC is a public-key algorithm technique that has been gaining popularity among constrained IoT devices. The popularity is due to using significantly smaller operands when compared to other public-key techniques such as RSA (Rivest Shamir Adleman). This paper shows the design, development, and evaluation of an application-specific secure communication architecture based on SRAM PUF technology and ECC for constrained IoT devices. More specifically, it introduces an Elliptic Curve Diffie-Hellman (ECDH) public-key based cryptographic protocol that utilizes PUF-derived keys as the root-of-trust for silicon authentication. Also, it proposes a design of a modular hardware architecture that supports the protocol. Finally, to analyze the practicality as well as the feasibility of the proposed protocol, we demonstrate the solution by prototyping and verifying a protocol variant on the commercial Xilinx Zynq-7000 APSoC device.

==> protAbkup.tex <==
%\setlength{\belowcaptionskip}{-10pt}
\begin{figure*}[t]
\hfill
\begin{minipage}[t][][b]{0.76\textwidth}
\begin{prot}
    \resizebox{\textwidth}{!} {
    \fbox{
        \pseudocode[codesize=\large]
        {%
        \textbf{(I) Enrollment of the device and the server} \< \< \\[0.2\baselineskip]
        \textbf{Trusted Third Party (TTP)}~has~SK_{TTP} \<\< \textbf{Device~(ID)} \\[0.1\baselineskip][\hline]
         \<\<\<\\ [-0.5\baselineskip]
         \<\<\pcln (x,~HD)~\gets PUF-enroll\\
         \<\<\pcln PK_{ID}\gets ~DH~\kgen(x) \\ %=xB
         \< \sendmessageleft * [6 cm] {\pcln ID, HD, PK_{ID} } \<\\
         \pcln \sigma_{ID} \gets \sig_{\sk_{TTP}}(ID, HD, PK_{ID}) \<\<\\
         \pcln Cert_{ID}=[ID, HD, PK_{ID}, \sigma_{ID}] \<\<\\
        \pcln Store(Cert_{ID})~in~cloud \<\<\\
        \< \sendmessageright * [6 cm]{\pcln PK_{TTP}} \<\\
         \<\< \pcln Store(PK_{TTP})\\
        \textbf{Trusted Third Party (TTP)}~has~SK_{TTP} \<\< \textbf{Server~(ID)} \\[0.1\baselineskip][\hline]
         \<\<\<\\ [-0.5\baselineskip]
         \<\<\pcln (SK_{server},PK_{server})\gets~DH~ \kgen \\
         \< \sendmessageleft * [6 cm] {\pcln ID, PK_{server} } \<\\
         \pcln \sigma_{ID} \gets \sig_{\sk_{TTP}}(ID, PK_{server}) \<\<\\
         \pcln Cert_{ID_{server}}=[ID, PK_{ID}, \sigma_{ID}] \<\<\\
         \< \sendmessageright * [6 cm]{\pcln Cert_{ID_{server}},PK_{TTP}} \<\\
         \<\< \pcln Store(Cert_{ID_{server}},SK_{server}, PK_{TTP})\\ %~in~NVM
         %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
         \textbf{(II) Key-agreement and Authentication}  \<\< \\[0.2\baselineskip]
         \textbf{Server}~has~PK_{TTP}~and~access~to~cloud \<\< \textbf{Device~(ID)}~has~PK_{TTP}  \\[0.1\baselineskip][\hline]
         \<\<\<\\ [-0.5\baselineskip] 
         \pcln Retrieve(Cert_{ID})~from~cloud\\
         \pcln \verify_{\pk_{TTP}}(Cert_{ID}) \\
         \< \sendmessageright * [6 cm]{\pcln Session~request,~HD,~Cert_{ID_{server}}} \<\\
         \<\<\pcln \verify_{\pk_{TTP}}(Cert_{ID_{server}})\\
                \<\< \pcln x~\gets PUF-reconstruct(HD)\\ 
         \pcln w=SK_{server}*PK_{ID} \<\<  \pcln w=x*PK_{server}\\
         \pcln \key~=KDF(w) \<\< \key~=KDF(w)  \\
        % [0.1\baselineskip] \pclb
        % \pcintertext [dotted] {Key Agreement complete} \\
         %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
       % \textbf{(III) Authentication}  \<\< \\[0.2\baselineskip]
         \pcln \text{Challenge-response handshake in both directions} \<\< %\\[0.01\baselineskip]
        %[0.05\baselines  kip] \pclb
        %\pcintertext [dotted] {Key-agreement and Authentication complete} \\
        }
     }%fbox
    }
\end{prot}
    \end{minipage}
\hfill
\begin{minipage}[t][][b]{0.23\textwidth}
%\vspace{0.0001cm}
\resizebox{\textwidth}{!}{
\begin{tabular}{|c|c|}
    \hline  %\cellcolor{headrBlue!20}
    \multicolumn{2}{|c|}{Protocol Legend}\\\hline
    $ID$ &  Device ID, 48 bits\\\hline
    $SK_{TTP}$ &  TTP's secret key, 256 bits\\\hline
    $PK_{TTP}$ &  TTP's public key, 256 bits\\\hline
    
    $x$ &  PUF-based secret key, 256 bits \\\hline
    $HD$ &  Helper data, 752 bytes \\\hline
    $PK_{ID}$ &  Device's Public Key, 256 bits\\\hline
    $\sigma_{ID}$ &  Digital signature, 256 bits\\\hline
   
    $SK_{server}$ & Server's secret key, 256 bits\\\hline
    $PK_{server}$ & Server's public key, 256 bits\\\hline
    $w, k$ &  Shared secret and key, 256 bits\\\hline
    
    $Cert_{ID}$ &  Device's Certificate  \\\hline
    $Cert_{ID_{server}}$ &  Certificate \\\hline
    
    
    $*$ &  Scalar multiplication \\\hline
    $KDF()$ &  Key Derivation Function \\\hline
    $Vf$ &  Signature Verification \\\hline

    
\end{tabular}}
\end{minipage}\hfill
\captionof{protocol}{Protocol based on \acf{DHKE} using \acf{PUF}-derived key. Variant A - \textit{Achieving mutual-authentication and low \acf{NVM} requirement using the cloud infrustructure.}}
\label{prot:variant_a}
\end{figure*}
